Learning to Bid Without Knowing your Value

We address online learning in complex auction settings, such as sponsored search auctions, where the value of the bidder is unknown to her, evolving in an arbitrary manner and observed only if the bidder wins an allocation. We leverage the structure of the utility of the bidder and the partial feedback that bidders typically receive in auctions, in order to provide algorithms with regret rates against the best fixed bid in hindsight, that are exponentially faster in convergence in terms of dependence on the action space, than what would have been derived by applying a generic bandit algorithm and almost equivalent to what would have been achieved in the full information setting. Our results are enabled by analyzing a new online learning setting with outcome-based feedback, which generalizes learning with feedback graphs. We provide an online learning algorithm for this setting, of independent interest, with regret that grows only logarithmically with the number of actions and linearly only in the number of potential outcomes (the latter being very small in most auction settings). Last but not least, we show that our algorithm outperforms the bandit approach experimentally and that this performance is robust to dropping some of our theoretical assumptions or introducing noise in the feedback that the bidder receives.

==> abstract.tex <==
We address online learning in complex auction settings, such as sponsored search auctions, where the value of the bidder is unknown to her, evolving in an arbitrary manner and observed only if the bidder wins an allocation. We leverage the structure of the utility of the bidder and the partial feedback that bidders typically receive in auctions, in order to provide algorithms with regret rates against the best fixed bid in hindsight, that are \emph{exponentially faster} in convergence in terms of dependence on the action space, than what would have been derived by applying a generic bandit algorithm and almost equivalent to what would have been achieved in the full information setting. Our results are enabled by analyzing a new online learning setting with outcome-based feedback, which generalizes learning with feedback graphs. We provide an online learning algorithm for this setting, of independent interest, with regret that grows only logarithmically with the number of actions and linearly only in the number of potential outcomes (the latter being very small in most auction settings). Last but not least, we show that our algorithm outperforms the bandit approach experimentally and that this performance is robust to dropping some of our theoretical assumptions or introducing noise in the feedback that the bidder receives.
%



==> compare-to-weed.tex <==
%
In this section we are going to show how our Outcome-Based feedback framework can be used in order to recover the result proved by Weed et al. \cite{WRP16} for adversarial online learning in repeated second price auctions. Suppose that in the second price auction, the maximum bids from other bidders $m_t = \max_{j \neq i} b_j$ for all the rounds form a grid, $\mathcal{L}_T$, in the bidding space $[0,1]$. \vsedit{Let $l^o=(m_t, m_{t'})$ be the widest interval in ${\cal L}_T$, such that there exists $b^* \in l^o$ with $b^*\in \argmax_{b \in [0,1]} \sum_{t=1}^T \E (v_t - m_t) \1 \{b>m_t\}$, i.e. $l^o$ contains an optimal fixed bid in hindsight. We denote with $\Delta^o$ the length of $l^o$.} 
\vsdelete{Observe also that the bids which guarantee that the bidder wins the item form a set generally, rather than being a single one and out of this set, we are picking the largest one. }
\vsdelete{This assumption about the grid of the bids of the opponents might seem unreasonable, but is indeed valid, as proved by Weed et at. in \cite{WRP16} when adversaries are oblivious. \cp{In the adaptive adversaries case, $\Delta^o$is the narrowest interval though.}} \vscomment{This sentence didn't make sense to me.}

Suppose we partition the bidding space of the learner into $\frac{1}{\epsilon}$ intervals of equal length $\epsilon$, for $\epsilon < \Delta^o$ and let $B$ denote this discretized bid space.
\vsedit{Since $b^*\in l^o$, any bid $b\in l^o$ is also optimal in-hindsight, since it achieves the same utility as $b^*$. Since $\Delta^o>\epsilon$, there must exist a bid $b_{\epsilon}^*\in B\cap l^o$. Thus $b_{\epsilon}^*$ is also optimal in hindsight. Hence, regret against the best fixed bid in $[0,1]$ is equal to regret against the best fixed bid in $B$. By our Theorem \ref{thm:outcome-based-main}, the latter regret is $4\sqrt{T\log(\nicefrac{1}{\epsilon})}$, which is exactly the same regret bound achieved by \cite{WRP16} with a more intricate adaptive discretization.
}
%
%
%
%
%
%
%
%
%
%
%
%

\vsedit{We note that all the above will require the %
discretization of our algorithm requires a choice of $\epsilon$ that depends on $\Delta^o$ and hence requires knowledge of $\Delta^o$ ahead of time. Similar to \cite{WRP16} (which also require knowledge of $\Delta^o$), the latter can be addressed by first replacing the definition of $\Delta^o$ with the more conservative quantity, which is the length of the smallest interval in ${\cal L}_T$ and then applying a standard doubling trick approach, where we keep track of an estimate of $\Delta^o$ and every time that $\Delta^o$ becomes smaller than our estimate we divide our current estimate in half and restart the algorithm. This will blow up the regret by only a constant factor.} %

%

\vsdelete{The benefit of our framework, however, is not that it can recover previously analyzed regret bounds, but rather that it can encapsulate the tools needed to analyze even more general cases. As an example of that, in this subsection we will discuss why the dynamic interval partitioning that Weed et al. describe in their paper would not work for cases more general than the second price auctions, by analyzing what would happen in a Sponsored Search Auction environment. The reason why the dynamic interval partitioning in the adversarial setup works is because at each timestep $i \in T$ either the bidder wins or loses the item auctioned, therefore, increases the interval space by at most 2 \footnote{Remember that when $m_t \in (x,y]$ then we break interval $(x,y]$ into two subintervals: $(x,m_t], (m_t,y]$, having each subinterval represent the continuous intervals where the bidder either wins or loses the item auctioned.}. However, in a Sponsored Search Auction there are $k$ available slots and $(k+1)$ allocation outcomes \footnote{With the extra outcome being the allocation of no slot.} at the end of each round and therefore, such a dynamic partitioning of the bidding space would create an exponential booming of intervals. Indeed, if we denote as $\pi_{\kappa,t}, \kappa \in \{1,\dots, k+1\}$ the payment after timestep $t$ that guarantees that the learner still gets allocated to slot $\kappa$ and if $\pi_{\kappa,t} \in (x_\kappa,y_\kappa]$, then with the dynamic partitioning algorithm after timestep $t$ the learner creates subintervals $(x_\kappa, \pi_{\kappa,t}], (\pi_{\kappa,t},y_\kappa]$ for every $\kappa \in \{1,\dots,k+1\}$. Thus, we are creating a total of $2^{k}$ new intervals at every timestep $t$. Observe now that the intervals that we create at every $t$ are going to be used as the arms for the multi-armed bandit problem at step $t+1$. Therefore, this dynamic partitioning would increase exponentially the number of arms and thus, result in much higher regret. 
}
\vscomment{I think we don't need this discussion here. It's obvious that our approach is more general than Weed by the many applications, so why try to show that their approach doesn't generalize. In fact it's not clear what the analogue of their partition is for multi-slot GSP. In fact, I think the right analogue wont be creating $2^k$ slots as you describe. It would just create intervals for each distinct threshold for each slot. Thus $(k+1)*T$ intervals. The reason is that any bid within such an interval is indistinguishable and that's what their interval partitioning is trying to accomplish.}
